EdgeMLBalancer: A Self-Adaptive Approach for Dynamic Model Switching on Resource-Constrained Edge Devices

The widespread adoption of machine learning on edge devices, such as mobile phones, laptops, IoT devices, etc., has enabled real-time AI applications in resource-constrained environments. Existing solutions for managing computational resources often focus narrowly on accuracy or energy efficiency, failing to adapt dynamically to varying workloads. Furthermore, the existing system lack robust mechanisms to adaptively balance CPU utilization, leading to inefficiencies in resource-constrained scenarios like real-time traffic monitoring. To address these limitations, we propose a self-adaptive approach that optimizes CPU utilization and resource management on edge devices. Our approach, EdgeMLBalancer balances between models through dynamic switching, guided by real-time CPU usage monitoring across processor cores. Tested on real-time traffic data, the approach adapts object detection models based on CPU usage, ensuring efficient resource utilization. The approach leverages epsilon-greedy strategy which promotes fairness and prevents resource starvation, maintaining system robustness. The results of our evaluation demonstrate significant improvements by balancing computational efficiency and accuracy, highlighting the approach's ability to adapt seamlessly to varying workloads. This work lays the groundwork for further advancements in self-adaptation for resource-constrained environments.

==> Sections/implementation-overview.tex <==
\section{Implementation Overview}

We implemented EdgeMLBalancer as a mobile application, designed to run on Android Devices. The application was developed using Android Studio \cite{b24}, with the primary algorithms written in Kotlin\footnote{\url{https://kotlinlang.org/}}. The TensorFlow Lite library\footnote{\url{https://www.tensorflow.org/resources/libraries-extensions}} was employed for on-device ML model inference, ensuring compatibility with edge-devices. The application integrates \textit{CameraX API}\footnote{\url{https://developer.android.com/media/camera/camerax}} for real-time video feed processing and \textit{MetricLogger} for monitoring and logging system metrics, including CPU usage, and model accuracy. The logging functionality write metrics to CSV file for later analysis. The source code, datasets, and ML models are available here.\footnote{\url{https://github.com/sa4s-serc/EdgeMLBalancer}}

